Parametric Complexity Bounds for Approximating PDEs with Neural Networks

Recent experiments have shown that deep networks can approximate solutions to high-dimensional PDEs, seemingly escaping the curse of dimensionality. However, questions regarding the theoretical basis for such approximations, including the required network size, remain open. In this paper, we investigate the representational power of neural networks for approximating solutions to linear elliptic PDEs with Dirichlet boundary conditions. We prove that when a PDE's coefficients are representable by small neural networks, the parameters required to approximate its solution scale polynomially with the input dimension $d$ and proportionally to the parameter counts of the coefficient networks. To this we end, we develop a proof technique that simulates gradient descent (in an appropriate Hilbert space) by growing a neural network architecture whose iterates each participate as sub-networks in their (slightly larger) successors, and converge to the solution of the PDE. We bound the size of the solution, showing a polynomial dependence on $d$ and no dependence on the volume of the domain.

==> sections/ErrorAnalysis/additional_helper_lemmas.tex <==
\section{Additional Helper Lemmas}
\begin{definition}[Angles between subspaces]
    \Tnote{TODO:Add definitions here}
\end{definition}
    
Assuming that $V = \Keigenfunctions$ and $\tilde{V} = \Keigenfunctionsapprox$ and 
$V_\perp = \spn\{\varphi_{k+1}, \ldots, \varphi_{\infty}\}$ 
and 
$V_\perp = \spn\{\tvarphi_{k+1}, \ldots, \tvarphi_{\infty}\}$
% $\tilde{V}_\perp = \spn\{\varphi_{k+1}, \ldots, \varphi_{\infty}\}$
We define 
$$
\cos \Theta(V, \hat{V}) 
= \inf_{\substack{x \in V, y \in \tilde{V} \\ \|x\|_{\l2} = 1 \\ \|y\|_{\l2} = 1}}
\langle x, y\rangle_{\l2}
$$
\Tnote{Cos here is defined with $\inf$ to match the $\sigma_{\min}$ in Andrej's paper definition.}
$$
\sin \Theta(V, \hat{V}) 
= \sup_{\substack{x \in V_\perp, y \in \tilde{V} \\ \|x\|_{\l2} = 1 \\ \|y\|_{\l2} = 1}}
\langle x, y\rangle_{\l2}
$$

\begin{align*}
    d_c(V, \tilde{V}) 
    &= \min_O\sup_{\substack{a \in \R^k \\ \sum_{i=1}^k a_i = 1}} \|\sum_{i=1}^k (O\varphi_i - \tvarphi_i)a_i\|_{\l2} \\
    &= \min_O \sup_{\substack{x \in V, y \in \tilde{V}\\ \|x\|_{\l2} = 1 \\ \|y\|_{\l2} = 1}} \|Oy - x\|_{\l2} \\
    &= \min_O \sup_{\substack{x \in V, y \in \tilde{V}\\ \|x\|_{\l2} = 1 \\ \|y\|_{\l2} = 1}} \sqrt{\|Oy - x\|^2_{\l2}} \\
    &= \min_O \sup_{\substack{x \in V, y \in \tilde{V}\\ \|x\|_{\l2} = 1 \\ \|y\|_{\l2} = 1}}
        \sqrt{\langle Oy, Oy\rangle_{\l2} + \langle x, x \rangle_{\l2} - 2\langle Oy, x \rangle_{\l2}}\\
    &= 2 \left( 1 - 
        \max_O \inf_{\substack{x \in V, y \in \tilde{V}\\ \|x\|_{\l2} = 1 \\ \|y\|_{\l2} = 1}} \sqrt{\langle Oy, x\rangle_{\l2}}
        \right) 
        \numberthis \label{eq:distance_final_form_but_one}
\end{align*}

Now, looking at the following term,
\begin{align*}
    \max_O \inf_{\substack{x \in V, y \in \tilde{V}\\ \|x\|_{\l2} = 1 \\ \|y\|_{\l2} = 1}} \langle Oy, x\rangle_{\l2}
    \geq \inf_{\substack{x \in V, y \in \tilde{V}\\ \|x\|_{\l2} = 1 \\ \|y\|_{\l2} = 1}} \langle y, x\rangle_{\l2}
    = \cos \Theta(V, \tilde{V})
    \numberthis \label{eq:max_cos_relation}
\end{align*}

Therefore from \eqref{eq:distance_final_form_but_one} and \eqref{eq:max_cos_relation} we have
\begin{align*}
    d_c(V, \tilde{V}) \leq \sqrt{2\left(1 - \cos\Theta(V, \tilde{V})\right)} = \|2\sin\frac{\Theta(V, \tilde{V})}{2}\|_2
\end{align*}

Further, we define $\sin \Theta(V, \tilde{V})$ as follows,
$$\sin \Theta(V, \tilde{V}) 
= 
\sup_{\substack{x \in V_\perp, y \in \tilde{V}\\ \|x\|_{\l2}\\ \|y\|_{\l2}}}\langle x, y\rangle_{\l2}$$

==> sections/ErrorAnalysis/error_analysis.tex <==
\section{Error Analysis}
\label{section:error_analysis_whole}
\red{
\textbf{TODO:}
\begin{itemize}
    \item multi-index cannot be $0$, increase the number there and change $\alpha$ to $\alpha-1$
\end{itemize}
}

\textbf{Notation}
The $n$ compositions of operator $L$ is denoted as 
$L^{(n)}:= \underbrace{L \circ L \circ \cdots \circ L}_{\text{n times}}$.
Further for given an operator $L$, we define a new operator
$L_{k}: \h \to \h$ where for all $x \in \Omega$ we have,
$(L_{k})u = -\sum_{ij}(\partial_k a_{ij})\partial_{ij}u - \sum_{ij}\partial_{ki}a_{ij}\partial_{j}u + \partial_k cu$.
\Tnote{Maybe use a generic notation here.}
\orange{Fill this up here}

\begin{theorem}
    Let $u^\star$ denote the solution to the PDE $Lu = f$,
    and $\tilde{u}^\star$ is the solution to the PDE $\tilde{L}u = \tilde{f}$,
    \begin{align*}
        \tilde{L}u \equiv -\divergence(\tilde{A}\nabla u) + \tilde{c} u = \tilde{f}
    \end{align*}
    Then there exists a constant $\epsilon^\star$
    such that $\|\tilde{u} - \tilde{u}^\star\| \leq \epsilon^\star$.
\end{theorem}
\begin{proof}
    First, we define a PDE $(Lu)(x) = \tilde{f}(x)$ for all $x \in \Omega$ and $u(x) = 0$ 
    for all $x \in \partial \Omega$ with solution denoted by $\tilde{u}$.
    Note that the following holds,
    \begin{align}
        \label{eq:breaking_of_difference_ustar_tilde_u}
        \|u^\star - \tilde{u}^\star\|_{\l2} \leq 
        \underbrace{\|u^\star - \tilde{u}\|}_{(i)}
        + \underbrace{\|\tilde{u}^\star - \tilde{u}\|_{\l2}}_{(ii)}
    \end{align}

    Using the fact that $u^\star = L^{-1}f$, we have the following,
    \begin{equation}
        \label{eq:difference_of_us}
        \|\tilde{u}^\star - \tilde{u}\|_{\l2} 
        = \|(\tilde{L}^{-1} - L^{-1})\tilde{f}\|_{\l2} 
        = \|(\tilde{L}^{-1}L - I)\tilde{u}\|_{\l2}
    \end{equation}
    Further, using \eqref{eq:tildeL_minus_L} from Lemma~\ref{lemma:inner_product_close}, 
    we have for all $u \in \h$,
    \begin{align*}
        &\langle (L - \tilde{L})u,u\rangle_{\l2} \leq \alpha \langle Lu, u\rangle_{\l2} \\
        \implies& \langle (L\tilde{L}^{-1} - I)\tilde{L}u,u\rangle_{\l2} \leq \alpha \langle Lu, u\rangle_{\l2} \\
        \implies& \langle (L\tilde{L}^{-1} - I)\tilde{f}, u \rangle_{\l2} 
            \leq \alpha \langle \tilde{f}, u \rangle_{\l2}\\
        \implies& \langle L\tilde{L}^{-1}\tilde{f}, u \rangle_{\l2} \leq (1 + \alpha)\langle \tilde{f}, u \rangle_{\l2}
        \numberthis \label{eq:LtildeL_inv_final}
    \end{align*}
    where $\tilde{f} \in \h$. Therefore we have,
    \begin{align}
        \label{eq:LtildeL_inv_operator_norm}
        \|L\tilde{L}^{-1}\|_2 
        = \sup_{v \in \h}\frac{\langle L\tilde{L}^{-1}v, v\rangle}{\|v\|^2_{\l2}}
        &\leq \sup_{v \in \h}\frac{(1 + \alpha)\langle v, v\rangle}{\|v\|^2_{\l2}} = (1 + \alpha)
    \end{align}
    Note that since $\|L\tilde{L}^{-1}\|_2 = \|\tilde{L}^{-1}L\|_2$, the following holds for all $u \in \h$,
    \begin{align*}
        &\langle \tilde{L}^{-1}Lu, u\rangle \leq (1 + \alpha)\|u\|_{\l2}^2 \\
        \implies& \langle (\tilde{L}^{-1}L -I)u, u\rangle \leq \alpha\|u\|_{\l2}^2 \\
        \implies& \|\tilde{L}^{-1}L -I\|_{\l2} \leq \alpha
        \numberthis \label{eq:tildeLinv_L_minus_I}
    \end{align*}
    Therefore, 
    using the inequality in \eqref{eq:tildeLinv_L_minus_I},
    \eqref{eq:difference_of_us} can be upper bounded to get,
    \begin{equation}
        \label{eq:tilde_u_star_tilde_u}
        \|\tilde{u}^\star - \tilde{u}\|_{\l2} \leq \alpha\|\tilde{u}\|_{\l2}
    \end{equation}

    \noindent In order to bound $\|u^\star - \tilde{u}\|_{\l2}$, we use the 
    result from \eqref{eq:operator_inequality} to get the following,
    \begin{align*}
        \|u^\star - \tilde{u}\|^2_{\l2} &\leq \frac{1}{\lambda_1}\langle L(u^\star - \tilde{u}), u^\star - \tilde{u}\rangle_{\l2} \\
        &= \frac{1}{\lambda_1} \langle f -\tilde{f}, u^\star - \tilde{u}\rangle_{\l2} \\ 
        &\leq \frac{1}{\lambda_1} \|f - \tilde{f}\|_{\l2}\|u^\star - \tilde{u}\|_{\l2} \\
        \implies \|u^\star - \tilde{u}\|_{\l2} &\leq \frac{1}{\lambda_1} \|f - \tilde{f}\|_{\l2}  
        \leq \frac{\epsilon_f}{\lambda_1} \numberthis \label{eq:ustar_utilde_difference}
    \end{align*}
    Therefore, combining results from
    \eqref{eq:tilde_u_star_tilde_u} and \eqref{eq:ustar_utilde_difference}, we have
    $$\|u^\star - \tilde{u}^\star\|_{\l2} \leq \alpha \|\tilde{u}\|_{\l2} + \frac{\epsilon_f}{\lambda_1} $$
    and $\epsilon^\star = \alpha \|\tilde{u}\|_{\l2} + \frac{\epsilon_f}{\lambda_1}$
\end{proof}
\Tnote{Should we remark on how small $\alpha$ should be??}

\begin{lemma}
    \label{lemma:inner_product_close}
    Given assumptions (i)-(iii), we define a linear elliptic PDE as
    $$\tilde{L}u \equiv (-\divergence(\tilde{A}\nabla u) + \tilde{c}u)(x) = f(x)$$
    for all $x \in \Omega$ and $u = 0$ for all $x = \partial \Omega$. 
    Then for all $u \in \h$ the following holds,
    \begin{equation}
        \label{eq:tildeL_minus_L}
        \langle (\tilde{L} - L)u, u\rangle \leq \alpha \langle Lu, u\rangle
    \end{equation}
    where $\alpha = \frac{\epsilon_A, \epsilon_c}{\min\{m, \eta\}}$.
\end{lemma}
\begin{proof}
   \begin{align*}
        \langle (L - \tilde{L})u, u\rangle 
        &= \int_\Omega \left((A - \tilde{A})\nabla u\cdot \nabla u + (c - \tilde{c})u^2\right) dx\\
        &\leq \left(\max_{ij}\|A_{ij} - \tilde{A}_{ij}\|_{\linf}\right)\|\nabla u\|^2_{\l2} + \|c - \tilde{c}\|_{\linf}\|u\|^2_{\l2}\\
        &\leq \max\{\epsilon_A, \epsilon_c\}\left(\|\nabla u\|^2_{\l2} + \|u\|^2_{\l2}\right)
        \numberthis \label{eq:final_LminusLtilde_innerp}
   \end{align*} 
   Further, note that
   \begin{align*}
       \langle Lu, u\rangle &= \int_{\Omega} A \nabla u \cdot \nabla u + cu^2 dx \\
       &\geq \min\{m, \eta\} \left(\|\nabla u\|^2_{\l2} + \|u\|^2_{\l2}\right)
       \numberthis \label{eq:final_L_lbd}
   \end{align*}
   Therefore combining \eqref{eq:final_LminusLtilde_innerp} and \eqref{eq:final_L_lbd} we have
   $$\langle (\tilde{L} - L)u, u\rangle \leq \alpha \langle Lu, u\rangle$$
    where $\alpha = \frac{\epsilon_A, \epsilon_c}{\min(m, \eta)}$.
\end{proof}


\orange{\subsection{Error analysis for $\tilde{f}$ and $\hat{f}$}}
\label{section:error_analysis_f_tilde_f}

\begin{lemma}[\blue{Operator Chain Rule}]
    Given an elliptic operator $L: \h \to \h$, 
    for all $v \in C^{\infty}(\Omega)$ we have the following
    \begin{equation}
        \label{eq:operator_chain_rule_relation}
        \nabla_k L^{(n)}u
            = \sum_{i=1}^n \left(L^{(n-i)}\circ L_k \circ L^{(i-1)}\right)(u)
            + L^{(n)}(\nabla_{k} u)
    \end{equation}
    \Tnote{Fix this part}
    \begin{equation}
        \label{eq:operator_chain_rule_relation}
        \nabla_{kl} L^{(n)}u
            = \sum_{i=1}^n \left(L^{(n-i)}\circ L_k \circ L^{(i-1)}\right)(u)
            + L^{(n)}(\nabla_{kl} u)
    \end{equation}
    where $\beta$ is a multi-index such that $|\beta|\leq 2$ and $L^{(0)} = I$.
\end{lemma}
\begin{proof}
   We show the proof using induction.
   For $n=1$ and  
    $|\beta|=1$, for all $k \in [d]$ we have 
   \begin{align*}
       \nabla_{k} (Lu) &= \nabla_{k}\left( -\divergence(A\nabla u) + cu\right)\\
       &= \nabla_k \left(-\sum_{ij}a_{ij} \partial_{ij} u - \sum_{ij}\partial_i a_{ij}\partial_j u + cu\right)\\
       &= \left(-\sum_{ij}a_{ij}\partial_{ij}(\partial_k u) - \sum_{ij}\partial_i a_{ij} \partial_j \partial_k u + c \partial_k u \right) + 
        \left(-\sum_{ij}\partial_k a_{ij} \partial_{ij}u - \sum_{ij} \partial_i \partial_k a_{ij} \partial_j u + \partial_k c u\right)\\
       &= L(\nabla_k u) + L_k u \numberthis \label{eq:operator_inequality_beta_1}
   \end{align*}
   Similarly for $|\beta| = 2$ and $k,l \in [d]$, 
   \begin{align*}
       \nabla_{kl} (Lu) &= \nabla_{kl} \left(-\divergence(A\nabla u) + cu\right)\\
       &= \nabla_{kl} \left(-\sum_{ij}a_{ij} \partial_{ij} u - \sum_{ij}\partial_i a_{ij}\partial_j u + cu\right)\\
       &= \left(-\sum_{ij}a_{ij}\partial_{ij}(\partial_{kl} u) - \sum_{ij}\partial_i a_{ij} \partial_j \partial_{kl} u + c \partial_{kl}u \right)
        +\left(-\sum_{ij}\partial_{k} a_{ij} \partial_{ij}\partial_l u 
            - \sum_{ij} \partial_i \partial_{k} a_{ij} \partial_j \partial_l u + \partial_{k} c \parital_l u\right)\\
        &+\left(-\sum_{ij}\partial_{l} a_{ij} \partial_{ij}\partial_k u 
            - \sum_{ij} \partial_i \partial_{l} a_{ij} \partial_j \partial_k u + \partial_{l} c \parital_k u\right)
        +\left(-\sum_{ij}\partial_{kl} a_{ij} \partial_{ij}u - \sum_{ij} \partial_i \partial_{kl} a_{ij} \partial_j u + \partial_{kl} c u\right)\\
       &= L(\nabla_{kl} u) + L_k (\nabla_l u) + L_l (\nabla_k u) + L_{kl} u \numberthis \label{eq:operator_inequality_beta_2}
   \end{align*}
   Therefore for $n=1$ we have that for $|\beta| \leq 2$, we have
   \begin{equation}
        \label{eq:operator_chain_rule_n_1}
       \nabla_{\beta} (Lu) = L(\nabla_\beta u) + L_\beta u
   \end{equation}
   \Tnote{This interchanging of multi-index and actual indices seems a bit weird with the notation.}
   
   Therefore, assuming that for all $k < n$, \eqref{eq:operator_chain_rule_relation} holds, i.e., we have,
   \Tnote{overloading $k$ here, change variable name}
   \begin{equation}
        \label{eq:operator_realtion_for_k}
        \nabla_\beta (L^{(k)}u)
            = \sum_{i=1}^k \left(L^{(k-i)}\circ L_\beta \circ L^{(i-1)}\right)(u)
            + L^{(k)}(\nabla_\beta u)
   \end{equation}
   For $k = n$ and $|\beta|=1$, using the result from \eqref{eq:operator_inequality_beta_1},
   for all $k \in [d]$ we have the following,
   \begin{align*}
       \nabla_k (L^{(n)}u) &= \nabla_k \left(L \circ L^{(n-1)}(u)\right)\\
       &= L\left(\nabla_k (L^{(n-1)} u)\right) + L_k\left(L^{(n-1)}u\right)\\
       &= L\left(\sum_{i=1}^{n-1} \left(L^{(n-1-i)}\circ L_{k} \circ L^{(i-1)}\right)u + L^{(n-1)}(\nabla_k u)\right) + L_k\left(L^{(n-1)}\right)u\\
       &= \sum_{i=1}^n \left(L^{(n-i)}\circ L_k \circ L^{(i-1)}\right)(u)
        + L^{(n)}(\nabla_k u) \numberthis \label{eq:operator_inequality_final_beta_1}
   \end{align*}
   \red{
   Further, similarly $k = n$ and $|\beta|=2$, using the result from \eqref{eq:operator_inequality_beta_2} we have
   for all $k,l \in [d]$ we have the following,
   \begin{align*}
       \nabla_{kl} (L^{(n)}u) &= \nabla_{kl} \left(L \circ L^{(n-1)}(u)\right)\\
       &= L\left(\nabla_{kl} (L^{(n-1)} u)\right) + L_{kl}\left(L^{(n-1)}u\right)\\
       &= L\left(\sum_{i=1}^{n-1} \left(L^{(n-1-i)}\circ L_{kl} \circ L^{(i-1)}\right)u + L^{(n-1)}(\nabla_{kl} u)\right) + L_{kl}\left(L^{(n-1)}\right)u\\
       &= \sum_{i=1}^n \left(L^{(n-i)}\circ L_{kl} \circ L^{(i-1)}\right)(u)
        + L^{(n)}(\nabla_{kl} u) \numberthis \label{eq:operator_inequality_final_beta_2}
   \end{align*}
   }
\end{proof}




\begin{lemma}[\blue{Upper Bound Order $1$}]
    \label{lemma:upper_bound_order_1}
    For all $u \in C^{\infty}(\Omega)$ or $u \in \h$, 
    then for all $k, l \in [d]$ the following upper bounds hold,
    \begin{equation}
        \label{eq:Lu_C_upper_bound}
        \|Lu\|_{\l2} \leq C \max_{\alpha:|\alpha| \leq 2} \|\partial^\alpha u\|_{\l2}
    \end{equation}
    \begin{equation}
        \label{eq:nabla_k_Lu_C_upper_bound}
        \|\nabla_k Lu\|_{\l2} \leq 2 \cdot C \max_{\alpha:|\alpha| \leq 3} \|\partial^\alpha u\|_{\l2}
    \end{equation}
    and
    \begin{equation}
        \label{eq:nabla_square_k_Lu_C_upper_bound}
        \|\nabla_{kl} Lu\|_{\l2} \leq 4 \cdot C \max_{\alpha:|\alpha| \leq 4} \|\partial^\alpha u\|_{\l2}
    \end{equation}
    where 
    $$C:=\green{(2d^2 + 1)}\max\left\{\max_{\alpha:|\alpha|\leq 3}\max_{i,j}\|\partial^{\alpha}a_{ij}\|_{\linf},
                 \max_{\alpha:|\alpha|\leq 2}\|\partial^\alpha c\|_{\linf}\right\}.$$
\end{lemma}
\begin{proof}
    We first begin calculating the upper bound for the quantity $\|Lu\|_{\l2}$
    \begin{align*}
        \|Lu\|_{\l2} &\leq \|-\sum_{i,j=1}^d a_{ij}\partial_{ij}u - \sum_{i,j=1}^d \partial_{i}a_{ij}\partial_j u + cu\|_{\l2}\\
        &\leq \underbrace{\green{(2d^2 + 1)}\max\left\{\max_{i,j}\|\partial_{i}a_{ij}\|_{\linf}, \max_{i,j}\|a_{ij}\|_{\linf}, \|c\|_{\linf}\right\}}_{C_1}
            \max_{\alpha:|\alpha|\leq 2}\|\partial^\alpha u\|_{\l2}\\
        &\leq C_1
            \max_{\alpha:|\alpha|\leq 2}\|\partial^\alpha u\|_{\l2}
        \numberthis \label{eq:Lu_C_1_upper_bound}
    \end{align*}

    In order to calculate $\|\nabla_k (Lu)\|_{\l2}$, we use the result from \eqref{eq:operator_inequality_beta_1},
    \begin{align*}
        \|\nabla_{k}(Lu)\|_{\l2} &\leq \|L_{k}u\|_{\l2} + \|L(\nabla_{k}u)\|_{\l2}\\
        &\leq \|-\sum_{i,j=1}^d\partial_{k}a_{ij}\partial_{ij}u - \sum_{i,j=1}^d\partial_{ik}a_{ij}\partial_{j}u + \partial_{k}cu\|_{\l2}\\
            &+ \| -\sum_{i,j=1}^da_{ij}\partial_{ijk}u - \sum_{i,j=1}^d\partial_ia_{ij} \partial_{jk}u + c\partial_{k}u\|_{\l2}\\
        &\leq \green{(2d^2 + 1)}\max\left\{\max_{\alpha:|\alpha|\leq 2}\max_{i,j}\|\partial^{\alpha}a_{ij}\|_{\linf}, \|\partial_{k} c\|_{\linf}\right\}
                \max_{\alpha:|\alpha|\leq 2}\|\partial^\alpha u\|_{\l2}\\
        &+ \green{(2d^2 + 1)}\max\left\{\max_{\alpha:|\alpha|\leq 1}\max_{i,j}\|\partial^{\alpha}a_{ij}\|_{\linf}, \|c\|_{\linf}\right\}
                \max_{\alpha:|\alpha|\leq 3}\|\partial^\alpha u\|_{\l2}\\
        \implies  \|\nabla_{k}(Lu)\|_{\l2}
        &\leq 2 \cdot \underbrace{\green{(2d^2 + 1)}\max\left\{\max_{\alpha:|\alpha|\leq 2}\max_{i,j}\|\partial^{\alpha}a_{ij}\|_{\linf},
                \max_{\alpha:|\alpha|\leq 1}\|\partial^\alpha c\|_{\linf}\right\}}_{C_2}
                \max_{\alpha:|\alpha|\leq 3}\|\partial^\alpha u\|_{\l2}\\
        &\leq 2 \cdot C_2 
                \max_{\alpha:|\alpha|\leq 3}\|\partial^\alpha u\|_{\l2}
        \numberthis \label{eq:nabla_k_Lu_C_2_upper_bound}
    \end{align*}
    Using the result from \eqref{eq:operator_inequality_beta_2}, we upper bound the quantity $\|\nabla_{kl}(Lu)\|_{\l2}$
    \begin{align*}
        \|\nabla_{kl}(Lu)\|_{\l2} &\leq \|L_{kl}u\|_{\l2} + \|L_k(\nabla_lu)\|_{\l2} + \|L_l(\nabla_k u)\|_{\l2} + \|L(\nabla_{kl}u)\|_{\l2}\\
        &\leq \|-\sum_{i,j=1}^d\partial_{kl}a_{ij}\partial_{ij}u - \sum_{i,j=1}^d\partial_{ikl}a_{ij}\partial_{j}u + \partial_{kl}cu\|_{\l2}\\
            &+ \| -\sum_{i,j=1}^d\partial_k a_{ij}\partial_{ij}\partial_lu - \sum_{i,j=1}^d\partial_i\partial_k a_{ij} \partial_{j}\partial_lu + \partial_k c\partial_{l}u\|_{\l2}\\
            &+ \| -\sum_{i,j=1}^d\partial_l a_{ij}\partial_{ij}\partial_ku - \sum_{i,j=1}^d\partial_i\partial_l a_{ij} \partial_{j}\partial_ku + \partial_l c\partial_{k}u\|_{\l2}\\
            &+ \| -\sum_{i,j=1}^da_{ij}\partial_{ijkl}u - \sum_{i,j=1}^d\partial_ia_{ij} \partial_{jkl}u + c\partial_{kl}u\|_{\l2}\\
        &\leq \green{(2d^2 + 1)}\max\left\{\max_{\alpha:|\alpha|\leq 3}\max_{i,j}\|\partial^{\alpha}a_{ij}\|_{\linf}, \|\partial_{kl} c\|_{\linf}\right\}
                \max_{\alpha:|\alpha|\leq 2}\|\partial^\alpha u\|_{\l2}\\
        &+ 2\green{(2d^2 + 1)}\max\left\{\max_{\alpha:|\alpha|\leq 2}\max_{i,j}\|\partial^{\alpha}a_{ij}\|_{\linf}, \|c\|_{\linf}\right\}
                \max_{\alpha:|\alpha|\leq 3}\|\partial^\alpha u\|_{\l2}\\
        &+ \green{(2d^2 + 1)}\max\left\{\max_{\alpha:|\alpha|\leq 2}\max_{i,j}\|\partial^{\alpha}a_{ij}\|_{\linf}, \|c\|_{\linf}\right\}
                \max_{\alpha:|\alpha|\leq 4}\|\partial^\alpha u\|_{\l2}\\
        \implies  \|\nabla_{kl}(Lu)\|_{\l2}
        &\leq 4 \cdot \underbrace{\green{(2d^2 + 1)}\max\left\{\max_{\alpha:|\alpha|\leq 3}\max_{i,j}\|\partial^{\alpha}a_{ij}\|_{\linf},
                \max_{\alpha:|\alpha|\leq 2}\|\partial^\alpha c\|_{\linf}\right\}}_{C_3}
                \max_{\alpha:|\alpha|\leq 4}\|\partial^\alpha u\|_{\l2}\\
        &\leq 4 \cdot C_3 
                \max_{\alpha:|\alpha|\leq 4}\|\partial^\alpha u\|_{\l2}
        \numberthis \label{eq:nabla_kl_Lu_C_3_upper_bound}
    \end{align*}
    Since $C_1 \leq C_2 \leq C_3$, we define $C:=C_3$ and therefore
    from equations \eqref{eq:Lu_C_1_upper_bound},
         \eqref{eq:nabla_k_Lu_C_2_upper_bound} and \eqref{eq:nabla_kl_Lu_C_3_upper_bound}
    the claim follows.
    
    Further, we note that from \eqref{eq:nabla_k_Lu_C_2_upper_bound}, we also have that
    \begin{equation}
        \label{eq:upper_bound_first_order_L_terms}
        \|L_k(u)\|_{\l2}, \|L(\nabla_k u)\|_{\l2} \leq C \max_{\alpha: |\alpha|\leq 3}\|\partial^\alpha u\|_{\l2}
    \end{equation}
    and similarly from \eqref{eq:nabla_kl_Lu_C_3_upper_bound} we have that,
    \begin{equation}
        \label{eq:upper_bound_second_order_L_terms}
        \|L_{kl}(u)\|_{\l2}, \|L_{k}(\nabla_l u)\|_{\l2},
        \|L_{l}(\nabla_k u)\|_{\l2}, \|L(\nabla_{kl}u)\|_{\l2}
        \leq C \max_{\alpha: |\alpha|\leq 4}\|\partial^\alpha u\|_{\l2}
    \end{equation}
\end{proof}



\begin{lemma}[\blue{Order $n$ Upper Bound}]
    \label{lemma:upper_bound_order_n}
    For all $u \in C^{\infty}(\Omega)$ or $u \in \h$
    and $k, l \in [d]$
    then for all $n \in \N$ we have the following upper bounds,
    \begin{equation}
        \|L^{(n)}u\|_{\l2} \leq (n!)^2 \cdot C^n \max_{\alpha: |\alpha| \leq n + 2} \|\partial^\alpha u\|_{\l2}
    \end{equation}
    \begin{equation}
        \|\nabla_k (L^{(n)}u)\|_{\l2} \leq (n+1) \cdot (n!)^2 \cdot C^n \max_{\alpha: |\alpha| \leq n + 2} \|\partial^\alpha u\|_{\l2}
    \end{equation}
    \begin{equation}
        \|\nabla_{kl} (L^{(n)}u)\|_{\l2} \leq ((n+1)!)^2 \cdot C^n \max_{\alpha: |\alpha| \leq n + 3} \|\partial^\alpha u\|_{\l2}
    \end{equation}
\end{lemma}
\begin{proof}
    We prove the following through induction. 
    Note that the case for $n=1$ follows from Lemma~\ref{lemma:upper_bound_order_1}, 
    where in order to bound $\|Lu\|_{\l2}$ we also use the 
    fact that $\max_{\alpha:|\alpha|\leq 2}\|\partial^\alpha u\|_{\l2} \leq \max_{\alpha:|\alpha|\leq 3}\|\partial^\alpha u\|_{\l2}$.
    
    Now, assume that for all $m \leq (n-1)$ the following holds,
    \begin{align*}
        \|L^{(m)}u\|_{\l2} &\leq (m!)^2 \cdot C^n \max_{\alpha: |\alpha| \leq m + 1} \|\partial^\alpha u\|_{\l2}\\
        \|\nabla_k (L^{(m)}u)\|_{\l2} &\leq (m+1) \cdot (m!)^2 \cdot C^n \max_{\alpha: |\alpha| \leq m + 2} \|\partial^\alpha u\|_{\l2}\\
        \|\nabla_{kl} (L^{(m)}u)\|_{\l2} &\leq ((m+1)!)^2 \cdot C^n \max_{\alpha: |\alpha| \leq m + 3} \|\partial^\alpha u\|_{\l2}
        \numberthis \label{eq:upper_bound_n_Lu_final}
    \end{align*}
    where, $C$ is defined in Lemma~\ref{lemma:upper_bound_order_1}.
    
    Therefore for $n$, the quantity $\|L^{(n)}u\|_{\l2}$, using \eqref{eq:Lu_C_upper_bound} we have
    \begin{align*}
        \|L^{(n)}u\|_{\l2} &= \|L(L^{(n-1)}u)\|_{\l2} \\
        &\leq C \cdot \max\left\{\|L^{(n-1)}u\|_{\l2}, \max_{i} \|\nabla_{i} (L^{(n-1)}u)\|_{\l2}, \max_{i,j}\|\nabla_{ij}(L^{(n-1)}u)\|_{\l2}\right\}\\
        &\leq C\cdot ((n-1)!)^2 \cdot C^{n-1} \max_{\alpha:|\alpha|\leq (n-1)+3}\|\partial^\alpha u\|_{\l2}\\
        \implies \|L^{(n)}u\|_{\l2} 
        &\leq ((n-1)!)^2 \cdot C^{n} \max_{\alpha:|\alpha|\leq n+2}\|\partial^\alpha u\|_{\l2}
    \end{align*}
    Further, for $k \in [d]$, using the inequality in \eqref{eq:operator_inequality_beta_1}
    the term $\|\nabla_k(L^{(n)}u)\|_{\l2}$ can be upper bounded as follows,
    \begin{align*}
        \|\nabla_{k}(L^{(n)}u)\|_{\l2} 
            &\leq \sum_{i=1}^n \left\|\left(L^{(n-i)}\circ L_k \circ L^{(i-1)}\right)(u)\right\|_{\l2} + \|L^{(n)}(\nabla_k u)\|_{\l2}\\
            &\leq (n) \cdot (n!)^2 \cdot C^n \max_{\alpha: |\alpha|\leq n+2}\|\partial^\alpha u\|_{\l2} 
                + (n!)^2 \cdot C^n \max_{\alpha:|\alpha|\leq n+2} \|\partial^\alpha u\|_{\l2}\\
            &\leq (n+1) \cdot (n!)^2 \cdot C^n \max_{\alpha: |\alpha|\leq n+2}\|\partial^\alpha u\|_{\l2} 
            \numberthis \label{upper_bound_n_nabla_final}
    \end{align*}
    Similarly, for $k,l \in [d]$ we use the inequality in \eqref{eq:operator_inequality_beta_2}
    \begin{align*}
        \|\nabla_{kl}(L^{(n)}u)\|_{\l2} 
        &\leq \sum_{\substack{i, j \\ i < j}}\left\|\left(L^{n-i} \circ L_k \circ L^{(j-i-1)} \circ L_l \circ L^{j-1}\right)u\right\|_{\l2}\\
        &+\sum_{\substack{i, j \\ i > j}}\left\|\left(L^{n-j} \circ L_k \circ L^{(i-j-1)} \circ L_l \circ L^{i-1} \right)u\right\|_{\l2}\\
        &+ \sum_{i}\left\|\left(L^{n-i} \circ L_{kl} \circ L^{i-1}\right)u\right\|_{\l2}
        + \|L^{(n-1)}(\nabla_{kl}u)\|_{\l2}\\
        &\leq n(n +1) \cdot (n!)^2 \cdot C^n \max_{\alpha:|\alpha|\leq n+2}\|\partial^\alpha u\|_{\l2} \\
        &+ n \cdot (n!)^2 \cdot C^n \max_{\alpha:|\alpha|\leq n+2}\|\partial^\alpha u\|_{\l2} 
        + C^n \max_{\alpha:|\alpha|\leq n+3}\|\partial^\alpha u\|_{\l2} \\
        \implies 
        \|\nabla_{kl}(L^{(n)}u)\|_{\l2} 
        &\leq \left((n+1)!\right)^2 \cdot C^n \max_{\alpha:|\alpha|\leq n+3}\|\partial^\alpha u\|_{\l2} \\
        \numberthis \label{upper_bound_n_nabla_square_final}
    \end{align*}
    Therefore from \eqref{eq:upper_bound_n_Lu_final}, \eqref{upper_bound_n_nabla_final} and \eqref{upper_bound_n_nabla_square_final}
    the claim follows.
\end{proof}


\begin{theorem}
    Consider that the function
    $\tilde{f} \in \Keigenfunctions$ can be approximated by a 
    neural network $\tilde{f}$ with $O(N_f)$ parameters,
    such that $\tilde{f} = \hat{f} + r$,
    where $r \in C^{\infty}(\Omega)$ and $\partial^\alpha r\|_{\l2} \leq C$ for all $|\alpha| \in \N$.
    Then the function $u_t$ can be approximated by a neural network $\hat{u}_t$ such that
    $\|u_t - \hat{u}_t\|_{\l2}$ is of the order 
    \textbf{\orange{Fill it up here!!}}
\end{theorem}

\begin{proof}
    For a given $t$, 
    we denote by $\hat{u}_t$ the neural network approximation 
    of the function $u_t$,
    and the function $r_t$ to denotes the error in the approximation such that, 
    $$\|r_t\|_{\l2} =  \|u_t - \hat{u}_t\|_{\l2}.$$
    Therefore, for $t=1$, using the update in \eqref{eq:update_equation_convergence_proof}, we have, 
    \begin{align*}
        r_1 &= u_1 - \hat{u}_1 \\
            &= u_0 - \eta \left(Lu_0 - \tilde{f}\right) - \left(u_0 - \eta \left(Lu_0 - \hat{f} - r\right) \right) \\
            &= \eta r \numberthis \label{eq:r_1_is_eta_r}\\
       \implies \|r_1\|_{\l2} &= \eta \|r\|_{\l2} \leq \eta \delta
    \end{align*}

    The update for $u_{t+1}$ is the following,
    \begin{align*}
        u_{t+1} &= u_t - \eta\left(Lu_t - \tilde{f}\right)\\
        u_{t+1} &= \hat{u}_t + r_t - \eta\left(L(\hat{u}_t + r_t) - \hat{f} - r\right)\\
        u_{t+1} &= \underbrace{\hat{u}_t - \eta\left(L(\hat{u}_t - \hat{f})\right)}_{\hat{u}_{t+1}} + r_t - \eta Lr_t - r
    \end{align*}
    Hence, we have the following to be true,
    \begin{align*}
        u_{t+1} - \hat{u}_{t+1} &= r_t - \eta Lr_t - r \\
        \implies r_{t+1} &= (I - \eta L)r_t - r\\
        \implies r_{t+1} &= (I - \eta L)^{(t)}r_1  + \sum_{i=0}^{t-1} (I - \eta L)^{(i)}r\\
        \implies r_{t+1} &= \eta(I - \eta L)^{(t)}r  + \sum_{i=0}^{t-1} (I - \eta L)^{(i)}r \qquad \text{from \eqref{eq:r_1_is_eta_r}} \end{align*}
    Where 
    $(I - \eta L)^{(k)} := \underbrace{(I - \eta L) \circ (I - \eta L) \circ \ldots (I - \eta L)}_{\text{$k$ times}} r$.
    Therefore for a $k \in \N$, using binomial expansion we can write the following,
    \begin{align*}
        (I - \eta L)^{(k)}r &= \sum_{i=0}^{(k)} {k\choose i}(\eta L)^{(i)}r \\
        \implies \|(I - \eta L)^{(k)}r\|_{\l2} 
        &= \left\|\sum_{i=0}^k {k\choose i}(\eta L)^{(i)}r\right\|_{\l2} \\
        &\leq \sum_{i=0}^k \left\|{k\choose i}\eta^i L^{(i)} r \right\|_{\l2}\\
        &\leq \sum_{i=0}^k (k\eta)^i \left\|L^{(i)} r \right\|_{\l2}\\
        &\leq \sum_{i=0}^k (k \eta)^i i! C^{i} \max_{\alpha:|\alpha|\leq i} \|\partial^\alpha u\|_{\l2} 
            \qquad \text{from Lemma~\ref{lemma:upper_bound_order_n}} \\
        &\leq \sum_{i=0}^k (ik \eta C)^i  \max_{\alpha:|\alpha|\leq i} \|\partial^\alpha u\|_{\l2}\\
        &\red{\leq \sum_{i=0}^k (k^2 \eta C)^i  \max_{\alpha:|\alpha|\leq k} \|\partial^\alpha u\|_{\l2}}\\
    \end{align*}
\end{proof}

==> sections/Proposition1/proposition1.tex <==
\begin{definition}[Gateaux Derivative]
    Let $G: \mathcal{U} \to \mathcal{V}$ be a function between two topological spaces. 
    For $x, h \in \mathcal{U}$ and $h \neq 0$, the Gateaux differential of $G$ at $x$ in the 
    direction of $h$ is defined as
    $$ F'[x](h) = \lim_{\epsilon \to 0} \frac{G(x + \epsilon h) - G(x)}{\epsilon}$$
\end{definition}


% With these preliminary notations, 
% we can define a bilinear form 
% that is induced by a linear PDE. 
% Towards that, the following proposition 
% follows from Definition~\ref{eq:main_pde}.
% (For completeness, we provide the proof 
% as Proposition \ref{proposition:weak_solution}, 
% though the result is standard.) 


% Having introduced these preliminaries, 
% we can now introduce the variational formulation of a linear PDE.
% % bilinear form of a linear PDE. 
% This form will prove useful because 
% under a reasonable set of assumptions 
% to be introduced in Section \ref{section:main_result},
% the unique solution $u^*$ of this formulation
% is the solution to the corresponding PDE.  
% Moreover, we will define a related bilinear form 
% % that will be convenient for developing our analysis.
% that we will use extensively in developing our analysis.


Having introduced these preliminaries, we now introduce 
some important concepts and formulations for a linear PDE,
which we will use extensively in developing our analysis.
\begin{proposition}
    % Consider Equation~\ref{eq:variational_formulation}, then the 
    For the PDE in Definition~\ref{eq:main_pde}, 
    given $f \in \l2$
    % following holds,
    the following hold:
    \begin{enumerate}
        % \item There exists a function $\bar{f} \in \h$ such that 
        % for all $v \in \h$,
        % $\langle f, v\rangle_{\l2} = \langle \bar{f}, v \rangle_{\l2}$.
        \item The solution $u^\star$ to the PDE is unique and obtained 
        as
        % $F[u] = \min_{u \in \h}\frac{1}{2}\|Lu - \bar{f}\|^2_{\hh}$
        % $$u^* = \mbox{argmin}_{u \in 
        $$u^\star = \argmin_{u \in 
        \h} F[u],\; \text{where}\;\;  F[u]= \frac{1}{2}\|Lu - \bar{f}\|^2_{\l2}.$$
        \item For all $v \in \h$, the Gateaux derivative of $F[u]$ at a point $u \in \h$ in the direction $v$
        is given by 
        $ F'[u](v) = \langle Lu - \bar{f}, v\rangle_{\l2}.$
        \item 
        $u^\star$ is the unique stationary point of $F$, that is $F'[u](v) = 0, \forall v \in \h$ if and only if $u = u^\star$.
        Equivalently, for all $v \in \h$ we have, 
        \begin{equation}
            \label{eq:variational_formulation}
        %   \langle Lu, v \rangle = \langle \bar{f}, v \rangle =(f, v),  \qquad \forall v \in \h
           \langle Lu, v \rangle_{\l2} = \langle \bar{f}, v \rangle_{\l2} = \langle f, v\rangle_{\l2},
        \end{equation}
        if and only if $u = u^\star$.
    \end{enumerate}
\label{p:maingd}    
\end{proposition}
\begin{proof}
    % First, we prove point 1.
    % For all $v\in \h$, let 
    % $l(v) := \langle f, v\rangle_{\l2}$ be a linear operator defined on $\h$. 
    % Note that from 
    % the 
    % Riesz representation theorem there exists a function $\bar{f} \in \h$ such that 
    % $l(v) = \langle \bar{f}, v\rangle_{\l2}$. 
    % This completes the proof.
    
    To get the result in 
    point 3,
    we calculate the Gateaux derivative of $F[u]$, \emph{i.e.},
    for a $v \in \h$,
    \begin{align*}
        F'[u](v) 
        =& \lim_{\epsilon \to 0}\frac{F[u + v] - F[u]}{\epsilon} \\
        =& \lim_{\epsilon \to 0}\frac{1}{2}\frac{\|L(u + \epsilon v) - \bar{f}\|_{\l2}^2 - \|Lu - \bar{f}\|_{\l2}^2}{\epsilon} \\
        =& \lim_{\epsilon \to 0}\frac{1}{2}\Bigg( \frac{\langle L(u + \epsilon v) - \bar{f}, L(u+ \epsilon v) - \bar{f} \rangle_{\l2}}{\epsilon} - \frac{\langle Lu - \bar{f}, Lu - \bar{f}\rangle}{\epsilon}\Bigg)\\
        =& \langle Lu - \bar{f}, Lv \rangle_{\l2}
    \end{align*}
    Using the fact that $L: \h \to \h$ and therefore $Lv \in \h$ (see Lemma~\ref{proposition:L_H01_H01}), we have that
    for all $v \in \h$ there exists a $v' \in \h$, such that any stationary point $u$ of $F$ will statisfy
    \Tnote{Added the fact that for every $v$ there exists a $v'$}
    \begin{align*}
        &F'[u](v) = \langle Lu - \bar{f}, v' \rangle_{\l2} = 0 \\
        \implies &\langle Lu, v' \rangle_{\l2}  = \langle \bar{f}, v' \rangle_{\l2}  \\
        \implies &\langle Lu, v' \rangle_{\l2} = \langle f, v'\rangle_{\l2} \qquad \text{using part (1)}.
    \end{align*}
    % \hl{Using the fact that $L: \h \to \h$ and therefore $Lv \in \h$, we have that}
    % for all $v \in \h$, the stationary point of $F$ will statisfy that,
    % \begin{align*}
    %     F'[u^\star](v) &= \langle Lu - \bar{f}, v \rangle_{\l2} = 0 \\
    %     \implies \langle Lu, v \rangle_{\l2}  &= \langle \bar{f}, v \rangle_{\l2}  \\
    %     \implies \langle Lu, v \rangle_{\l2} &= \langle f, v\rangle_{\l2} \qquad \text{using part (1)}.
    % \end{align*}
    Note that (\ref{eq:variational_formulation}) has a unique solution (referred to as $u^\star$).
    The proof for this is standard 
    % and is included in the Appendix 
    (see Proposition~\ref{proposition:unique_solution_proof} in the Appendix).
    Therefore, since the stationary point of $F[u]$ 
    satisfies (\ref{eq:variational_formulation}) 
    and we know that the solution to the equation is unique,
    % it implies that 
    % we establish that
    it follows that
    $F[u]$ has a unique stationary point ($u^\star$).
    % \noindent
    % The proof for uniqueness of the solution $u^\star$ is standard 
    % and included in Appendix~\ref{proposition:unique_solution_proof}.
\end{proof}

The first part of the proposition states 
that we can find a function $\bar{f} \in \h$
where $f_{|\partial \Omega} = 0$ 
such that the $\l2$ inner products are equal. 
This ensures that the minimization defined in Part 2 
is expressed over functions 
that satisfy the boundary condition 
for our PDE (Definition~\ref{eq:main_pde})---i.e., 
that they lie in $\h$---and 
hence the solution $u^\star \in \h$ as well.
Note that equation (\ref{eq:variational_formulation}) 
is also referred to as the \emph{variational formulation} 
for the PDE in Definition~\ref{eq:main_pde}.

==> sections/archive.tex <==
\begin{proof}
    We denote $\tilde{L} = \left(I - \frac{2}{\lambda_k + \lambda_1}L\right)$.
    We note that the $\tilde{L}$ has the same eigenfunctions as $L$ and 
    from Lemma~\ref{lemma:bounded_operator_norm} (part 2) we have that 
    \begin{equation}
        \label{eq:appendix_operator_norm_ineq}
      \sup_{\substack{v \in \h\\ v \in \Keigenfunctionsmath} } \frac{|\langle \tilde{L}v, v \rangle|}{\|v\|_{\l2}^2} 
      = \frac{\lambda_k - \lambda_1}{\lambda_k + \lambda_1}
    \end{equation}
    Hence, we have
    \begin{align*}
        \|\tilde{L}u\|_{\l2} = \frac{\|\tilde{L}u\|^2_{\l2}}{\|\tilde{L}u\|_{\l2}} = \left\langle \tilde{L}u, \frac{\tilde{L}u}{\|\tilde{L}u\|_{\l2}} \right\rangle_{\l2}
    \end{align*}
    Consider $v := \frac{\tilde{L}u}{\|\tilde{L}u\|_{\l2}}$, note that $v \in \Keigenfunctionsmath$ since $u \in \Keigenfunctionsmath$.
    Substituting $v$ in the above equation we get,
    \begin{align*}
        \|\tilde{L}u\|_{\l2} &= \left\langle \tilde{L}u, \frac{\tilde{L}u}{\|\tilde{L}u\|_{\l2}} \right\rangle\\
        &= \langle \tilde{L}u, v\rangle_{\l2} \\
        &\leq  \sup_{\|v\|_{\l2} = 1} \langle \tilde{L}u, v \rangle \\ 
        &\leq \sup_{\|v\|_{\l2} = 1} \frac{\lambda_k - \lambda_1}{\lambda_k + \lambda_1} \|u\|_{\l2} \|v\|_{\l2} 
        \qquad 
        \text{(using (\ref{eq:appendix_operator_norm_ineq}) and Lemma~\ref{lemma:general_operator_norm_upper_bound_elliptic_operator}})\\
        \\
        &\leq \frac{\lambda_k - \lambda_1}{\lambda_k + \lambda_1} \|u\|_{\l2}
        \qedhere
    \end{align*}
\end{proof}

\begin{lemma}
    \label{lemma:general_operator_norm_upper_bound_elliptic_operator}
    Let $\mathcal{L}$ be a symmetric elliptic operator, 
    with $\{(\gamma_i, \phi_i)\}_{i=1}^k$
    begin the first $k$ (eigenvalue, eigenfunction) pairs.
    Then for functions $g, h \in \Keigenphis$,
    the following holds,
    \begin{align}
        \langle \mathcal{L}g, h \rangle_{\l2} \leq \gamma_k \|g\|_{\l2}\|h\|_{\l2},
    \end{align}
    where $$\gamma_k = \sup_{\substack{h \in \h \\ h \in \Keigenfunctionsmath}} \frac{|\langle \mathcal{L}h, h\rangle|}{\|h\|_{\l2}}$$
\end{lemma}
\begin{proof}
    Since $g, h \in \Keigenphis$, 
    we have $g = \sum_{i=1}^k d_i \phi_i$,
    where $d_i = \langle g, \phi_i\rangle, \forall i \in \{1, \ldots, k\}$ 
    and similarly $h = \sum_{i=1}^k e_i \phi_i$,
    where $e_i = \langle h, \phi_i\rangle, \forall i \in \{1, \ldots, k\}$.
    
    Therefore using the fact that 
    $\gamma_1 \leq \gamma_2, \cdots, \gamma_k$ and $\gamma_1 > 0$
    (see \cite{evans1998partial}, Section 6.5), 
    we have
    % (see Remark~\ref{remark:laplacian_remark} - in fact $\lambda_1 > \frac{1}{C_p}$) we have, 
    \begin{align*}
        \langle \mathcal{L}g, h \rangle_{\l2} &= \left\langle \mathcal{L}\left(\sum_{i=1}^kd_i \phi_i \right), \left(\sum_{i=1}^k e_i \phi_i\right) \right\rangle_{\l2} \\
            &= \left\langle \sum_{i=1}^k \gamma_i d_i \phi_i,\sum_i^k e_i \phi_i\right\rangle_{\l2} \\
            &\leq  \sum_{i}^k|\gamma_i||d_i| |e_i| \qquad 
            (\because \langle \phi_i, \phi_i\rangle_{\l2} = 1, \; \&\; \langle \phi_i, \phi_j \rangle_{\l2} = 0 \text{ when $i \neq j$})\\
            &\leq \gamma_k \sum_{i=1}^k |d_i||e_i| \qquad (\because 0 < \gamma_1 \leq \gamma_2 \ldots \leq \gamma_k)\\
            &\leq \gamma_k \sqrt{\left(\sum_{i=0}^k d_i^2\right)}\sqrt{\left(\sum_{i=0}^ke_i^2\right)} \qquad
            \left(\because \sum_{i}a_ib_i \leq \sqrt{\sum_i a_i^2}\sqrt{\sum_i b_i^2}\right)\\
            &= \gamma_k \|g\|_{\l2} \|h\|_{\l2}
            \qedhere
    \end{align*}
\end{proof}

\begin{lemma}
    \label{lemma:proof_for_upper_bounding_operator_norm_k_eigenfunctions}
    % Consider an operator $L: \h \to \h$ with eigenfunctions $\{\varphi_i\}_{i=1}^\infty$ and eigenvalues $\lambda_1 \leq \lambda_2 \cdots $
    Let $L$ be the operator defined in Definition~\ref{definition:eigenvalue_eigenfunctions}.
    Then for functions $u, v \in \Keigenfunctionsmath$
    the following holds,
    \begin{align}
        \langle Lu, v \rangle_{\l2} \leq \lambda_k \|u\|_{\l2}\|v\|_{\l2}
    \end{align}
    where $$\lambda_k = \sup_{\substack{v \in \h \\ v \in \Keigenfunctionsmath}} \frac{|\langle Lv, v\rangle|}{\|v\|_{\l2}}$$
\end{lemma}
\begin{proof}
    %Note that a function $g \in \h$ can also be written as $g = \sum_{i=1}^\infty \mu_i \varphi_i$, where $\mu_i = \langle g, \varphi_i\rangle_{\l2}$.
    %Further, the norm is also defined as $\|g\|^2_{\l2} := \sum_{i=1}^\infty \mu^2_i$.
    
    Since $u, v \in \Keigenfunctionsmath$, we have
    $u = \sum_{i=1}^k d_i \varphi_i$ where $d_i = \langle u, \varphi_i\rangle, \forall i \in \{1, \ldots, k\}$ and similarly 
    $v = \sum_{i=1}^k e_i \varphi_i$ where $e_i = \langle v, \varphi_i\rangle, \forall i \in \{1, \ldots, k\}$.
    
    Therefore using the fact that $\lambda_1 \leq \lambda_2, \cdots, \lambda_k$ and $\lambda_1 > 0$
    (see \cite{evans1998partial}, section 6.5), we have
    % (see Remark~\ref{remark:laplacian_remark} - in fact $\lambda_1 > \frac{1}{C_p}$) we have, 
    \begin{align*}
        \langle Lu, v \rangle_{\l2} &= \left\langle L\left(\sum_{i=1}^kd_i \varphi_i \right), \left(\sum_{i=1}^k e_i \varphi_i\right) \right\rangle_{\l2} \\
            &= \left\langle \sum_{i=1}^k \lambda_i d_i \varphi_i,\sum_i^k e_i \varphi_i\right\rangle_{\l2} \\
            &\leq  \sum_{i}^k|\lambda_i||d_i| |e_i| \qquad 
            (\because \langle \varphi_i, \varphi_i\rangle_{\l2} = 1, \; \&\; \langle \varphi_i, \varphi_j \rangle_{\l2} = 0 \text{ when $i \neq j$})\\
            &\leq \lambda_k \sum_{i=1}^k |d_i||e_i| \qquad (\because 0 < \lambda_1 \leq \lambda_2 \ldots \leq \lambda_k)\\
            &\leq \lambda_k \sqrt{\left(\sum_{i=0}^k d_i^2\right)}\sqrt{\left(\sum_{i=0}^ke_i^2\right)} \qquad
            \left(\because \sum_{i}a_ib_i \leq \sqrt{\sum_i a_i^2}\sqrt{\sum_i b_i^2}\right)\\
            &= \lambda_k \|u\|_{\l2} \|v\|_{\l2}
    \end{align*}
\end{proof}


\textbf{For the proof in Lemma~\ref{lemma:convergence_proof}, we have}

\textcolor{orange}{provide some context/transition, or break into a separate subsection? The current form is a bit abrupt.}

\begin{align*}
    u_{t+1} - u^\star &= \left(I - \frac{2}{\lambda_k + \lambda_1}L\right) (u_t - u^\star) \\
    \left\langle u_{t+1} - u^\star, u_{t+1} - u^\star\right\rangle_{\l2} &=
        \left\langle \left(I - \frac{2}{\lambda_k + \lambda_1}L\right) (u_t - u^\star), u_{t+1} - u^\star \right\rangle_{\l2}\\
    \left\| u_{t+1} - u^\star\right\|^2_{\l2} &\leq \frac{\lambda_k -\lambda_1}{\lambda_k + \lambda_1} \|u_t - u^\star\|_{\l2} \|u_{t+1} - u^\star\|_{\l2}\\
    \implies \left\| u_{t+1} - u^\star\right\|_{\l2} &\leq \frac{\lambda_k -\lambda_1}{\lambda_k + \lambda_1}  \|u_t - u^\star\|_{\l2}
\end{align*}


\begin{lemma}
    \label{lemma:proof_for_upper_bounding_operator_norm_k_eigenfunctions}
    given an operator $l: \h \to \h$ 
    such that 
    $$\sup_{\substack{v \in \h \\ v \in \keigenfunctionsmath}} 
        \frac{\left|\left\langle \left(i - \frac{2}{\lambda_k + \lambda_1}l\right)v, v \right\rangle\right|}{\|v\|_{\l2}} = \frac{\lambda_k - \lambda_1}{\lambda_k + \lambda_1}$$
    then for all function $v \in \keigenfunctionsmath$, 
    $$\left\| \left(i - \frac{2}{\lambda_k + \lambda_1}l\right) v \right\|_{\l2}
        \leq \frac{\lambda_k - \lambda_1}{\lambda_k + \lambda_1} \|v\|_{\l2}
    $$
\end{lemma}
\begin{proof}
    denoting 
    $v = \sum_{i=1}^k d_i\varphi_i$
    where $d_i = \langle v, \varphi_i\rangle_{\l2}$, 
    further 
    \begin{align*}
    \left\| \left(i - \frac{2}{\lambda_k + \lambda_1}l\right) v \right\|^2_{\l2} 
    &= \left\|\left(i - \frac{2}{\lambda_1 + \lambda_k}l\right)
        \sum_{i=1}^k d_i\varphi_i\right\|^2_{\l2} \\
    &= \left\|\sum_{i=1}^k \tilde{\lambda}_i\varphi_id_i\varphi_i\right\|^2_{\l2} \\
    \end{align*}
    % denoting 
    % $$u_t = \sum_{i=1}^k d^t_i\varphi_i$$ where $d^t_i = \langle u_t, \varphi_i\rangle_{\l2}$
    % similarly denoting $u_{t+1}$, and $\tilde{u}$ we can re-write the above equation as,
    % {\small
    % \begin{align*}
    %     (\sum_{i=1}^k d^{t+1}_i  - \sum_{i=1}^k \tilde{d}_i) \varphi_i &= \left(i - \frac{2}{\lambda_k + \lambda_1}l\right)(\sum_{i=1}^k d^t_i - \sum_{i=1}^k \tilde{d})\varphi_i\\
    %     &= \sum_{i=1}^k\tilde{\lambda}_i(\sum_{i=1}^k d^t_i - \sum_{i=1}^k \tilde{d})
    % \end{align*}
    % }
    % here $\{\tilde{\lambda}_i\}_{i=1}^k$ are the eigenvalues for the operator $(i - \frac{2}{\lambda_k + \lambda_1}l)$.
\end{proof}

\subsection{Proof of Lemma~\ref{lemma:identity_approximation}}
\begin{proof}
    We first define a function $\hat{f}: \bar{\Omega} \rightarrow \R$: 
    \begin{align*}
        \hat{f}(x) = 
            \begin{cases}
                f(x), \qquad x \in \Omega \\
                0, \qquad  \hfill x \in \partial \Omega 
            \end{cases}
    \end{align*}
    Furthermore, let $\mathbb{I}_g(x):= \mathbb{I}\{g(x)\}$, so that
    \begin{equation}
        \label{eq:f_hat}
        \hat{f}(x) = f(x) \cdot \left(1 - \mathbb{I}_g(x)\right)
    \end{equation}
    By Lemma~\ref{lemma:activation_approximation}, for the choice of $\gamma$ in the theorem statement, we have 
    $$\forall r > 0, \int_{B_d(r)} \left(\mathbb{I}\{y = 0\} - \sigma(y) \right)^2 dy \leq \frac{\delta}{\|f\|_{\l2}}$$
    
    Further given that 
    \begin{equation}
        \tilde{f}(x) = f(x) \cdot \left(1 - \sigma(g(x))\right)
    \end{equation}
    We have: 
    \begin{align*}
      \|\hat{f} - \tilde{f}\|_{\l2}^2 
            &= \|f \cdot \left(\mathbb{I}_g - \sigma \circ g\right)\|_{\l2}^2 \quad \mbox{(Cauchy-Schwartz)} \\
            &\leq \|f\|_{\l2}^2 \|\mathbb{I}_g - \sigma \circ g\|_{\l2}^2 \\
            &= \|f\|_{\l2}^2 \int_\Omega \left(\mathbb{I}\{g(x) = 0\} - \sigma(g(x))\right)^2 dx \\
            &\leq \|f\|_{\l2}^2 \int_{B_d(r)} \left(\mathbb{I}\{g(x) = 0\} - \sigma(g(x))\right)^2 dx  \quad (\because \bar{\Omega} \subseteq B(r))\\
            &\leq \|f\|_{\l2}^2 \frac{\delta}{\|f\|^2_{\l2}}
            \leq \delta
    \end{align*}
    % \Anote{Update above with bug fixed} 
    Therefore, 
    \begin{align*}
        \|f - \tilde{f}\|_{\l2} &\leq \|f - \hat{f}\|_{\l2}+ \|\hat{f} - \tilde{f}\|_{\l2}  \\
        &\leq \|\hat{f} - \tilde{f}\|_{\l2} \\
        &\leq \delta
    \end{align*}
    Where we have $\|f - \hat{f}\|_{\l2} = 0$ by construction. 
    This proves point (2). 
    
    The neural network to approximate the function $\tilde{f}$
    can be constructed by appending the network $\phi_f$ with $\phi_g$.
    Following Lemma~\ref{lemma:lemma_operations} the final neural network 
    $\phi_{\tilde{f}}$ can be approximated in $O(N_g + N_f)$ parameters, which gives us point (3). 
    
    For (1), by construction, it's clear $\tilde{f}_{|\partial \Omega = 0}$. Further, given that $f \in \l2$ and $\|f - \tilde{f}\|_{\l2} \leq \delta$, we have $\tilde{f} \in \l2$. 
    % \Anote{Why is this needed?} 
    Finally,  for all $x \in \Omega$ we have
    \begin{align*}
        \nabla \tilde{f}(x) &= \nabla f(x) \cdot (1 - \sigma(g(x))) - \frac{1}{2\gamma^2}f(x) \sigma'(g(x)) \nabla g(x)\\
        % \|\nabla \tilde{f}\|_{\l2} &\leq \|1 - \sigma\circ g\|_{L^\infty(\Omega)}\|\nabla f\|_{\l2} + \frac{1}{2\gamma^2}\|f\|_{L^\infty(\Omega)} \|\sigma'\circ g\|_{L^\infty(\Omega)} \|\nabla g\|_{\l2} \\
        \|\nabla \tilde{f}\|_{\l2} &\leq \|1 - \sigma\circ g\|_{\infty}\|\nabla f\|_{\l2} + \|\sigma'\circ g\|_{\infty} \|f\|_{\l2}\|\nabla g\|_{\l2} \\
        &\leq \|\nabla f\|_{L^2(\Omega)} + \frac{1}{\gamma}\exp\left(-\frac{1}{2}\right)\|f\|_{\l2}\|\nabla g\|_{\l2} \leq \infty
    \end{align*}
    Where we use that $\|1 - \sigma(y)\|_{\infty} \leq 1$ for all $y \in \R$ and that $\|\sigma'(y)\|_{\infty} = \frac{1}{\gamma}\exp(-1/2)$.
    Therefore as both $\|\nabla \tilde{f}\|_{\l2} \leq \infty$ it implies that $\tilde{f}\in \h$ and proves (i).
    
    
    % \Anote{Last inequality is wrong. You dropped the $ \|1 - \sigma(y(\|_{L^\infty(\Omega)}\|$ term -- we should say in the assumptions this is bounded, and plug in the bound here.} which gives (1). 
    As a side remark, note that such a construction also verifies the fact that the $\h$ space is dense in $\l2$.
\end{proof}

\subsubsection{Continuous approximation of Identity Function}
\begin{lemma}
    \label{lemma:activation_approximation}
    Consider a function $g: B_d(r) \rightarrow \R$, where $B_d(r) := \{x: x \in \R^d, \|x\| \leq r\}$.
    Given the identity function $\mathbb{I}\{y = 0\}$ and a function $\sigma(y) = \exp(y^2/2\gamma^2)$ for all $y \in \R$,
    there exists a $\gamma' > 0$ such that for all $\gamma \leq \gamma'$, we have
    \begin{equation}
        \label{eq:integral_over_sphere}
        \int_{B_d(r)} \left(\mathbb{I}\{g(x) = 0\} - \sigma(g(x))\right)^2 dx \leq \delta.
    \end{equation}
\end{lemma}
\begin{proof}
    We first simplify the above expressions,
    \begin{align*}
        \int_{B_d(r)} \left(\mathbb{I}\{g(x) = 0\} - \sigma(g(x))\right)^2 dx &= \int_{B_d(r)\backslash \partial \Omega} \left(\sigma(g(x))\right)^2 dx 
        + \int_{\partial \Omega}\left(1- \sigma(g(x))\right)^2 dx   \\
        &= \int_{B_d(r)} (\sigma(g(x))^2 dx
    \end{align*}
    Here we are using the fact that $\int_{B_d(r) \backslash \partial \Omega} f(x) dx = \int_{B_d(r)} f(x) dx$ because $\partial \Omega$ is a measure zero set.
    
    Reparameterizing with $x$ by $(\theta, x_d)$ such that $dx = dx_d d\theta$ where $d\theta$ is an element of $d-1$ dimensional ball and $x_d \in [-r, r]$.
    \begin{align*}
        \int_{B_d(r)} \sigma(g(x))^2 dx 
        &= \int_{B_d(r)} \exp\left(-\frac{2g(x)^2}{2 \gamma^2}\right) dx \\
        &= \int_{\theta}\left\{\int_{-r}^r \exp\left(-\frac{g(\theta, x_d)^2}{\gamma^2}\right) dx_d \right\}d\theta\\
        &\leq \int_{\theta}\left\{\int_{-\infty}^\infty \exp\left(-\frac{g(\theta, x_d)^2}{\gamma^2}\right) dx_d \right\}d\theta\\
        &\leq \int_{\theta} \sqrt{\pi}\gamma d\theta\\
        &\leq \sqrt{\pi} \gamma \mbox{vol}(B_{d-1}(r))
    \end{align*}
    Hence, here $\gamma' = \frac{\delta}{\sqrt{\pi}\mbox{vol}(B_{d-1}(r))}$ and for all $\gamma \leq \gamma'$ 
    the integral in (\ref{eq:integral_over_sphere}) will be bounded.
\end{proof}

\subsection{Helper Lemmas for Section \ref{section:network_approximation}}
\begin{lemma}[Backpropagation~\cite{rumelhart1986learning}]
    \label{thm:backpropagation}
    Consider neural network $f:\R^m \rightarrow \R$ with depth $l$ and $N$ parameters,
    then there exists a neural of size $O(l + N)$ that calculates the gradient 
    $\frac{df}{di}$ for all $i \in [m]$.
\end{lemma}

\medskip
\begin{lemma}[Operations on Neural Network functionals]
    \label{lemma:lemma_operations}
    Given neural networks $f:\Omega \rightarrow \R$, $g: \Omega \rightarrow \R$,
    with $N_f$ and $N_g$ parameters respectively, 
    the operations 
    $f(x) + g(x)$ and $f(x) \cdot g(x)$ can
    be represented by neural networks of size $O(N_f + N_g)$,
    and square activation functions.
\end{lemma}
\begin{proof}
    For \emph{Addition}, there exists a network $h$ containing both networks $f$ and $g$ as subnetworks and an extra layer to 
    compute the addition between their outputs. Hence, the total number of parameters in such a network will be $O(N_f + N_g)$.

    For \emph{Multiplication}, consider the operation $f(x) \cdot g(x) = \frac{1}{2}\left(\left(f(x) + g(x)\right)^2 - f(x)^2 - g(x)^2\right)$.
    Then following the same argument as for addition of two networks, we can construct a network $h$ containing
    both networks and square activation function. 
\end{proof}

While the representation result in the above theorem is shown using
square activation, we refer to \cite{yarotsky2017error} 
for approximation results with ReLU activation. 
The scaling with respect to the number of parameters in the network
remains the same.

==> sections/operations_on_nn_functionals.tex <==


